Robust 3D Object Detection from LiDAR-Radar Point Clouds via Cross-Modal Feature Augmentation

This paper presents a novel framework for robust 3D object detection from point clouds via cross-modal hallucination. Our proposed approach is agnostic to either hallucination direction between LiDAR and 4D radar. We introduce multiple alignments on both spatial and feature levels to achieve simultaneous backbone refinement and hallucination generation. Specifically, spatial alignment is proposed to deal with the geometry discrepancy for better instance matching between LiDAR and radar. The feature alignment step further bridges the intrinsic attribute gap between the sensing modalities and stabilizes the training. The trained object detection models can deal with difficult detection cases better, even though only single-modal data is used as the input during the inference stage. Extensive experiments on the View-of-Delft (VoD) dataset show that our proposed method outperforms the state-of-the-art (SOTA) methods for both radar and LiDAR object detection while maintaining competitive efficiency in runtime. Code is available at https://github.com/DJNing/See_beyond_seeing.

==> section/introduction.tex <==
\section{Introduction}

Robust 3D object recognition and localization are crucial for autonomous driving systems, especially in urban environments. Ranging sensors like LiDAR and radar have become increasingly popular for this purpose due to their capability for depth sensing and immunity to lighting conditions.


While advances are witnessed in LiDAR- \cite{pointpillar, pointrcnn, yang2019std, liu2020tanet, shi2020pv, shi2020points, zhang2022not, yang20203dssd, yin2021center, noh2021hvpr} and radar-based 3D object detection \cite{bansal2020pointillism, vod}, each of them comes with intrinsic limitations.

LiDAR sensors can provide dense point clouds with informative geometry, but they lack per-point semantic information. Even though some LiDAR sensors can output point-level intensity values \cite{kitti, caesar2020nuscenes}, they are often inconsistent across semantic labels as lidar intensity is complexly determined by the distances between objects and LiDAR, rather than the object class alone \cite{chazette2016principle}. Due to the lack of semantic information, far objects or occluded objects with incomplete shapes or the insufficient number of points will be difficult for LiDAR to detect \cite{xu2021spg}. 
On the other side, 4D radars recently emerged as a promising automotive sensor against bad weather \cite{vod, meyer2019automotive}. While their point clouds suffer from point sparsity and low data fidelity, these radars can provide rich semantic features like Radar Cross Section (RCS) and the (Doppler) velocity. Unlike LiDAR intensity, RCS is a distance-independent measurement uniquely determined by the object material and reflection angle. The Doppler velocity measures the moving speed of a detected point relative to the ego vehicle. Benefiting from the rich semantic information provided by RCS and velocity measurements,  fairly reasonable 3D object performance can be achieved by less than $400$ points per scan even in complex urban environments \cite{vod}, while most of the objects contain less than 10 points per scan. 

The complementariness between these two sensors motivates us to explore the following question - \emph{Is it possible for one ranging sensor to learn to `imagine the lacking bits' from another heterogeneous ranging sensor so that it can later individually detect objects beyond its comfort zone?} 
For example, since both model inputs are point clouds, can we let a radar detection model learn from a LiDAR detection model to improve object detection robustness and vice versa? Indeed, due to the cost consideration, many low-end autonomous vehicles are only equipped with either radars or LiDARs. It is thus valuable to train a \emph{single-modal} detection model from the \emph{multimodal} data collected by pilot vehicles equipped with both sensors, yet dispatch the trained models on low-end vehicles equipped with only one of them.

This essentially requires us to address a cross-modal learning problem. Prior arts achieve cross-modal learning via hallucination for feature augmentation \cite{xu2017learning, saputra2020deeptio, hoffman2016learning, lezama2017not, choi2017learning} or knowledge distillation \cite{zheng2022boosting, yuan2022x, gupta2016cross, ren2021learning} for backbone refinement.
Traditionally, the hallucination network is trained separately with raw input data to provide extra information for specific tasks.  Consequently, the performance improvement of the framework depends entirely on the hallucination quality.

More recently, \cite{zheng2022boosting} leverages knowledge distillation to learn multi-modal information to improve a single-modal network. This method guides the backbone for better feature extraction but limits extra performance gain from hallucination features. Besides, this guidance only applies from the more robust modal-modal network to the weaker single-modal network. 

Unlike prior arts, in this work, we aim to realize simultaneous feature augmentation and backbone refinement by a new cross-modal hallucination framework.
Besides, to avoid information loss on sparse radar points and maintain runtime efficiency, we follow the point-based single shot detector architecture in our design. 
Notably, we target a framework agnostic to learning directions so that it can be applied to either hallucination direction between LiDAR and radar point clouds. 
To this end, we introduce multi-level alignment in this framework. 
The first one is space-level instance alignment which exploits instance co-locatiocentress different sensory data. 
Due to the discrepancy between sensory data and measurement noise from radar, it is difficult to establish fine-grained point-to-point matches between sensors. 
Thus, we employ an instance feature aggregation module that moves points to their corresponding object center to generate more comprehensive instance-level features.  By doing so, points belonging to the same instance in different modalities will be positioned near the instance center, which eases the effort for cross-modal matching.
The second one is feature-level alignment which is carried out by two learned non-linear mapping functions to project features from both modalities to a shared latent space respectively, which optimizes the training by closing the domain gap between modalities. 
With both spatial and feature alignment, our backbone can extract better intra-modality features via cross-modal learning and hallucinate inter-modality features to improve detection robustness, especially on hard samples (see Fig.~\ref{fig:open_fig}). 

% Summary
% In summary, our contributions are as follows:
% \begin{itemize}
% % \vspace{-0.5e}
%     \item Our method is the first object detection work from point clouds by utilizing cross-modal hallucination. Our method distinguishes itself in simultaneous backbone refinement and feature-level hallucination.
%     \item We introduce spatial and feature-level alignment to resolve the intrinsic measurement differences between LiDAR and radar point clouds to establish correct cross-modal supervision signals.
%     \item Our method outperforms previous state-of-the-art (SOTA) methods in 3D object detection, which we demonstrate on the public View-of-Delft dataset in both LiDAR and radar object detection tasks.
% \end{itemize}

\begin{figure}[t!]
    \centering
    \begin{subfigure}[h]{0.9\linewidth}
    \includegraphics[width=\linewidth]{figure/open_fig/proposed_method.pdf}
    \caption{Proposed method for 4D radar object detection}
    \label{fig:proposed_method}
    \end{subfigure}
    \begin{subfigure}[h]{0.45\linewidth}
    \includegraphics[width=\linewidth]{figure/open_fig/centerpoint.pdf}
    \caption{Centerpoint}
    \label{fig:open_fig_ctp}
    \end{subfigure}
    \begin{subfigure}[h]{0.45\linewidth}
    \includegraphics[width=\linewidth]{figure/open_fig/pp.pdf}
    \caption{Pointpillar}
    \end{subfigure}
    \begin{subfigure}[h]{0.45\linewidth}
    \includegraphics[width=\linewidth]{figure/open_fig/pvrcnn.pdf}
    \caption{PV-RCNN}
    \end{subfigure}
    \begin{subfigure}[h]{0.45\linewidth}
    \includegraphics[width=\linewidth]{figure/open_fig/ours.pdf}
    \caption{Ours}
    \label{fig:open_fig_ours}
    \end{subfigure}
    \caption{Fig.~\ref{fig:proposed_method} illustrates the proposed method with the 4D radar input as an example. Fig.~\ref{fig:open_fig_ctp} - Fig.~\ref{fig:open_fig_ours} are the visualization of radar detection in the same scene of different methods. Ground truth boxes are denoted in \textcolor{gt}{red}, the wrong detections are denoted in \textcolor{step_1}{yellow} and the correct detections are denoted in \textcolor{det}{green}. RGB images are \textbf{only used for visualization}. }
    \label{fig:open_fig}
%    \vspace{-5pt}
    \vspace{-2em}
\end{figure}

